Simultaneously Learning Stochastic and Adversarial Bandits with General Graph Feedback

The problem of online learning with graph feedback has been extensively studied in the literature due to its generality and potential to model various learning tasks. Existing works mainly study the adversarial and stochastic feedback separately. If the prior knowledge of the feedback mechanism is unavailable or wrong, such specially designed algorithms could suffer great loss. To avoid this problem, \citet{erez2021towards} try to optimize for both environments. However, they assume the feedback graphs are undirected and each vertex has a self-loop, which compromises the generality of the framework and may not be satisfied in applications. With a general feedback graph, the observation of an arm may not be available when this arm is pulled, which makes the exploration more expensive and the algorithms more challenging to perform optimally in both environments. In this work, we overcome this difficulty by a new trade-off mechanism with a carefully-designed proportion for exploration and exploitation. We prove the proposed algorithm simultaneously achieves $\mathrm{poly} \log T$ regret in the stochastic setting and minimax-optimal regret of $\tilde{O}(T^{2/3})$ in the adversarial setting where $T$ is the horizon and $\tilde{O}$ hides parameters independent of $T$ as well as logarithmic terms. To our knowledge, this is the first best-of-both-worlds result for general feedback graphs.

==> proof.tex <==
% %!TEX root =  main.tex
\section{Appendix}
% \section{Bar Graph Mentioned in Section \ref{sec:discuss}}



% a\begin{lemma}\label{lem:key:concen}
% For any arm $i \in V$ and time $t<\tau$, in the adversarial setting, we have with probability at least $1-\delta$,
% \begin{align*}
%     \abs{ \tilde{H}_{t}(i) -H_{t}(i) } \le \sqrt{ 4\bracket{ \frac{|D|}{t^2}\sum_{s=1}^{\min\set{t,\tau'_i}} \frac{1}{\gamma_s} + \frac{ |D| \cdot \max\set{t-\tau'_i, 0} }{\gamma_t \tau'_i t }  }\log \frac{t}{\delta} + \frac{5|D|^2 }{\gamma_t^2 \min\set{t^2, {\tau'_i}^2 } }\log^2 \frac{t}{\delta} }\,.
% \end{align*}
% Moreover, in the stochastic setting, with probability at least $1-\delta$,
% \begin{align*}
%     \abs{ \tilde{H}_{t}(i)- \mu_{i}  } \le \sqrt{ 4\bracket{ \frac{|D|}{t^2}\sum_{s=1}^{\min\set{t,\tau'_i}} \frac{1}{\gamma_s} + \frac{ |D| \cdot \max\set{t-\tau'_i, 0} }{\gamma_t \tau'_i t }  }\log \frac{t}{\delta} + \frac{5|D|^2 }{\gamma_t^2 \min\set{t^2, {\tau'_i}^2 } }\log^2 \frac{t}{\delta} }\,.
% \end{align*}
% \end{lemma}

% \begin{proof}[Proof of Lemma \ref{lem:key:concen}]

\subsection{Proof of Lemma \ref{lem:key:concen}}
The proof of the two inequalities is similar, here we mainly focus on the adversarial setting. 

In each round $t$, let $\cF_t$ be the history of observations. 
Define 
\begin{align*}
    X_{t}(i) = \tilde{r}_{t}(i) - r_{t}(i)=r_{t}(i)\bracket{ \frac{\bOne{i \in N^{\mathrm{out}}(I_t)}}{ \sum_{j\in N^{\mathrm{in}}(i)  } p_{s}(j)  } - 1  } \,. 
\end{align*}
Note that $(X_{s}(i))_{1 \le s \le t}$ is a martingale difference sequences. According to the algorithm, at each time $t<\tau$, 
\begin{align*}
    \sum_{j\in N^{\mathrm{in}}(i)  } p_{t}(j) \ge \frac{\gamma_t}{|D|} \bOne{ t\le \tau'_i } + \frac{\gamma_t \tau'_i}{|D|t} \bOne{ t>\tau'_i } \,.
\end{align*}
Thus $\abs{X_{t}(i)} \le \max\set{ \frac{|D|}{\gamma_t}, \frac{|D| t}{\gamma_t \tau'_i } } \le \frac{|D|}{\gamma_t} \max\set{1, \frac{t}{\tau'_i}} $ and
\begin{align*}
  \sum_{s=1}^t \EE{ X_{s}(i)^2 \mid \cF_{s-1} } \le \sum_{s=1}^{\min\set{t,\tau'_i}}\frac{|D|}{\gamma_s}
+ \sum_{s=\tau'_i}^{t}  \frac{|D| s}{ \gamma_s \tau'_i } \le \sum_{s=1}^{\min\set{t,\tau'_i}}\frac{|D|}{\gamma_s}
+ \frac{t|D|}{\gamma_t \tau'_i}\cdot \max\set{t-\tau'_i, 0}\,,
\end{align*}
where the last inequality holds since $\gamma_t$ decreases with the increase of $t$ by choosing $\gamma_t = (K^2 |D|)^{1/3} t^{-1/3}$. According to Lemma \ref{lem:tech:concen}, we have with probability at least $1-\delta$
\begin{align*}
    \sum_{s=1}^t X_{s}(i) \le \sqrt{ 4\bracket{ \sum_{s=1}^{\min\set{t,\tau'_i}}\frac{|D|}{\gamma_s}
+ \frac{t|D|}{\gamma_t \tau'_i}\cdot \max\set{t-\tau'_i, 0} }\log \frac{t}{\delta}  + \frac{5|D|^2}{\gamma_t^2} \max\set{1, \frac{t^2}{{\tau'_i}^2}} \log^2 \frac{t}{\delta}  } \,,
\end{align*}
and further
\begin{align*}
    \abs{ \tilde{H}_{t}(i) - H_{t}(i) } \le \sqrt{ 4\bracket{\frac{|D|}{t^2} \sum_{s=1}^{\min\set{t,\tau'_i}}\frac{1}{\gamma_s}
+ \frac{|D|}{\gamma_t \tau'_i t}\cdot \max\set{t-\tau'_i, 0} }\log \frac{t}{\delta}  + \frac{5|D|^2}{\gamma_t^2 \min\set{t^2, {\tau'_i}^2} } \log^2 \frac{t}{\delta}  } \,,
\end{align*}
since $\tilde{H}_{t}(i) - H_{t}(i) = \frac{1}{t} \sum_{s=1}^t X_{s}(i)$. 

% \end{proof}



\subsection{Proof of Lemma \ref{lem:sto:pullTime}}
% \begin{proof}[Proof of Lemma \ref{lem:sto:pullTime}]

Let $Z_{s,i}(p)\sim \mathrm{Bernoulli}(p)$ for time $s=1,2\ldots,t$, $i\in V$. Then $\forall i,t$, $T_i(t) = \sum_{s=1}^t Z_{s,i}(p_{s}(i))$. 
% \begin{align*}
%     T_i(t) = \sum_{s=1}^t Z_{s,i}(p_{s}(i)) \,.
%     % =  \sum_{s=1}^t Z_{s,i}\bracket{ (1-\gamma_s)\cdot p_{s,A}(i) + \gamma_s \cdot p_{s,D}(i) }\,.
% \end{align*}
Define $X_{s}(i) = Z_{s,i}(p_{s}(i)) - p_{s}(i) $. We have $\abs{X_{s}(i)} \le 1$ and 
\begin{align*}
    \sum_{s=1}^t \EE{X_{s}(i)^2 \mid \cF_{s-1} }
    % \le& \sum_{s=1}^{\tau_i}(1-\gamma_s)\cdot p_{s,A}(i) + \sum_{s=1}^{\tau_i^D} \gamma_s \cdot p_{s,D}(i) + \sum_{s=\tau_i^D}^t \gamma_s\cdot \frac{u_i\tau_i^D}{s} \\
    \le& \tau_i + \sum_{s=1}^{\tau_i^D}\gamma_s + \sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s} \,.
\end{align*}
According to Lemma \ref{lem:tech:concen}, with probability at least $1-\delta$, 
\begin{align*}
    T_i(t)  &\le \tau_i + \sum_{s=1}^{\tau_i^D}\gamma_s + \sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s} + \sum_{s=1}^t X_{s}(i)  \\
    &\le \tau_i + \sum_{s=1}^{\tau_i^D}\gamma_s + \sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s}  \\
    +&\sqrt{ 4\bracket{ \tau_i + \sum_{s=1}^{\tau_i^D}\gamma_s + \sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s} }\log \frac{T}{\delta} + 5\log^2 \frac{T}{\delta} } \,.
\end{align*}
% \end{proof}





% \subsection{Regret Analysis in the Adversarial Setting}

 

% \begin{theorem}\label{thm:adv}
% In the adversarial setting, let $i^* \in \argmax_{i\in V}G_{\tau}(i)$ be one of the optimal arms in the first $\tau$ rounds. Then with probability at least $1-\delta$, 
% \begin{align*}
%     \EE{Reg(T)} =& \EE{\max_{i\in V}\sum_{t=1}^T r_{t}(i) - r_{t}(I_t) }\\
%     \le & \EE{\sum_{t=1}^{\tau} r_{t}(i^*) - r_{t}(I_t) } + \EE{\max_{i\in V}\sum_{t=\tau+1}^T r_{t}(i) - r_{t}(I_t) } \le O\bracket{K^{2/3} |D|^{1/3} T^{2/3} \sqrt{\log\frac{T}{\delta}}} \,.
% \end{align*}

% \end{theorem}


% \begin{proof}
% According to \citet[Theorem 2]{alon2015online}, $\EE{\max_{i\in V}\sum_{t=\tau+1}^T r_{t}(i) - r_{t}(I_t) } \le O\bracket{ (|D|\log K)^{1/3}T^{2/3} }$. In the following, we mainly focus on the first $\tau$ rounds. 
% \begin{align}
%     \EE{\sum_{t=1}^{\tau} r_{t}(i^*) - r_{t}(I_t) } =& \sum_{t=1}^{\tau} \bracket{ r_{t}(i^*) - \sum_{i\in V} p_{t}(i) r_{t}(i) }  \notag \\
%     =& \sum_{t=1}^{\tau} \bracket{ r_{t}(i^*) - \sum_{i\in V} \gamma_{t}p_{t,D}(i) \cdot r_{t}(i) -  \sum_{i\in V} (1-\gamma_{t})p_{t,A}(i)\cdot  r_{t}(i) }  \notag \\
%     =& \sum_{t=1}^{\tau} \gamma_t \sum_{i\in V} p_{t,D}(i) \bracket{ r_{t}(i^*)-r_{t}(i) } +  \sum_{t=1}^{\tau} (1-\gamma_t) \sum_{i\in V} p_{t,A}(i) \bracket{ r_{t}(i^*)-r_{t}(i) } \notag\\
%     \le& \sum_{t=1}^{\tau} \gamma_t + \sum_{t=1}^{\tau}  \sum_{i\in V} p_{t,A}(i) \bracket{ r_{t}(i^*)-r_{t}(i) } \notag \\
%     \le& \sum_{t=1}^{\tau} \gamma_t + \sum_{i\in V} \sum_{t=1}^{\min\set{\tau_i,\tau}}   \bracket{ r_{t}(i^*)-r_{t}(i) } \label{eq:adv:since:updateA} \\
%     \le & \sum_{t=1}^{\tau} \gamma_t + \sum_{i\in V} \bracket{ \bOne{i\notin A_{\tau}}\cdot \tau_i  \bracket{ H_{\tau_i}(i^*)-H_{\tau_i}(i) } + \bOne{i\in A_{\tau}}\cdot \tau  \bracket{ H_{\tau}(i^*)-H_{\tau}(i) } } \notag \\
%     \le & \sum_{t=1}^{\tau} \gamma_t + \sqrt{ 256K^2|D| \sum_{t=1}^{\tau}\frac{1}{\gamma_t} \log \frac{T}{\delta} + \frac{320K^2|D|^2}{\gamma_{\tau}^2 }\log^2 \frac{T}{\delta} } \label{eq:adv:since:arm:bound} \\
%     \le& (K^2|D|)^{1/3}\bracket{1+\int_{1}^{\tau}t^{-1/3}dt } \notag \\
%     & + \sqrt{ 256K^{4/3}|D|^{2/3}\bracket{\tau^{1/3} +\int_{1}^{\tau} t^{1/3}dt } \log \frac{T}{\delta} + 320K^{2/3}|D|^{4/3}\tau^{2/3}\log^2 \frac{T}{\delta}} \label{eq:adv:since:SumAndGamma} \\
%     \le& O\bracket{ K^{2/3}|D|^{1/3}\tau^{2/3}
%     \sqrt{\log\frac{T}{\delta} }}\notag  \,,
% \end{align}
% where Eq.\eqref{eq:adv:since:updateA} holds according to Algorithm \ref{alg}, Eq.\eqref{eq:adv:since:arm:bound} comes from Lemma \ref{lem:adv:arm:bound} and Eq.\eqref{eq:adv:since:SumAndGamma} holds since $\gamma_t =(K^2|D|)^{1/3}t^{-1/3}$ and $\sum_{t=a}^b\gamma_t \le \max_{t\in[a,b]}\gamma_t + \int_{a}^{b}\gamma_t dt$. 

% \end{proof}












% \begin{lemma}\label{lem:adv:arm:bound}
% For any arm $i$ such that $i \notin A_{\tau-1}$, we have at time $\tau_{i}-1$, 
% \begin{align*}
%     H_{\tau_i-1}(i^*) - H_{\tau_i-1}(i) \le 8\sqrt{ \frac{4|D|}{(\tau_i-1)^2} \sum_{s=1}^{\tau_i - 1} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i - 1}^2 (\tau_i - 1)^2}\log^2 \frac{T}{\delta} } \,.
% \end{align*}
% Similarly, for any arm $i \in A_{\tau-1}$, at time $\tau-1$,
% \begin{align*}
%     H_{\tau-1}(i^*) - H_{\tau-1}(i) \le 8\sqrt{ \frac{4|D|}{(\tau-1)^2} \sum_{s=1}^{\tau - 1} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau - 1}^2 (\tau - 1)^2}\log^2 \frac{T}{\delta} } \,.
% \end{align*}

% \end{lemma}

% \begin{proof}
% For arm $i \notin A_{\tau-1}$, Eq.\eqref{eq:alg:delete:condition} does not hold at time $\tau_i-1$, which means
% \begin{align}
%       \tilde{H}_{\tau_i-1 }(i^*)-  \tilde{H}_{\tau_i-1 }(i) \le \max_{j\in A_{\tau_i-1}} \tilde{H}_{\tau_i-1 }(j)-  \tilde{H}_{\tau_i-1 }(i) \le 6\sqrt{ \frac{4|D|}{(\tau_i-1)^2} \sum_{s=1}^{\tau_i - 1} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i - 1}^2 (\tau_i - 1)^2}\log^2 \frac{T}{\delta} }  \label{eq:adv:arm1}\,,
% \end{align}
% where the first inequality holds according to Lemma \ref{lem:adv:optimalIsNotDelete}. 

% Besides, according to Algorithm \ref{alg}, since both $i^*$ and $i$ are in $A_{\tau_{i}-1}$, it holds that $\tau'_i > \tau_i-1$ and $\tau'_{i^*} > \tau_i-1$. Thus based on Lemma \ref{lem:key:concen}, 
% \begin{align}
%     \tilde{H}_{\tau_i-1}(i^*)-  \tilde{H}_{\tau_i-1}(i) &\ge H_{\tau_i-1 }(i^*)-H_{\tau_i-1}(i) - \radius_{\tau_i-1}(i^*) - \radius_{\tau_i-1}(i) \notag\\
%     &= H_{\tau_i-1}(i^*)-H_{\tau_i-1}(i) - 2\sqrt{ \frac{4|D|}{(\tau_i-1)^2} \sum_{s=1}^{\tau_i - 1} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i - 1}^2 (\tau_i - 1)^2}\log^2 \frac{T}{\delta} } \label{eq:adv:arm2} \,.
% \end{align}
% Combining Eq.\eqref{eq:adv:arm1} and \eqref{eq:adv:arm2}, we can obtain the first inequality in Lemma \ref{lem:adv:arm:bound}. Similar arguments hold at time $\tau-1$ for arm $i \in A_{\tau-1}$ to get the second inequality.  

% \end{proof}





% \begin{lemma}\label{lem:adv:optimalIsNotDelete}
% At time $\tau-1, i^* \in A_{\tau-1}$. 
% \end{lemma}
% \begin{proof}
% Denote $I^* \in \argmax G_{\tau-1}(i) $ as one of the optimal arm till $\tau-1$. Then for any arm $i \notin A_{\tau-1}$, we have
% \begin{align*}
%      &G_{\tau-1}(I^*) -  G_{\tau-1}(i) \\
%     =& G_{\tau-1}(I^*) - \tilde{G}_{\tau-1}(I^*) + \tilde{G}_{\tau-1}(I^*) - \tilde{G}_{\tau-1}(i) + \tilde{G}_{\tau-1}(i) - G_{\tau-1}(i) \\
%     =& (\tau-1)\cdot \bracket{ H_{\tau-1}(I^*) - \tilde{H}_{\tau-1}(I^*) + \tilde{H}_{\tau-1}(I^*) - \tilde{H}_{\tau-1}(i) + \tilde{H}_{\tau-1}(i) - H_{\tau-1}(i) }\\
%     \ge & \bracket{\tau-1}\cdot \bracket{-\radius_{\tau-1}(I^*)-\radius_{\tau-1}(i) +\tilde{H}_{\tau-1}(I^*) - \tilde{H}_{\tau-1}(i)}  > 0  
% \end{align*}
% where the last inequality holds since Eq.\eqref{eq:alg:detect:adv} in Algorithm \ref{alg} is not satisfied at $\tau-1$. 

% Above all, any previously deleted arm $i \notin A_{\tau-1}$ is worse than $I^*$, thus we can conclude that $i^* \in A_{\tau-1}$ holds. 
% \end{proof}









% \subsection{Regret Analysis in the Stochastic Setting}

% \begin{theorem}\label{thm:sto}
% With probability at least $1-\delta$, 
% \begin{align*}
%     Reg(T) = \sum_{t=1}^T \mu_{i^*} - \mu_{I_t} \le O\bracket{ |D|^2 \cdot \max_{j:j\neq i^*}\bracket{ \frac{\log T/\delta}{\Delta_j^2} }^{3/2}  } \,. 
% \end{align*}
% \end{theorem}

% \begin{proof}
% Based on the result of Lemma \ref{lem:sto:neverStartExp}, the Exp3.G algorithm is never started in the stochastic setting. Thus the regret can be bounded by
% \begin{align*}
%     Reg(T) =& \sum_{i\neq i^*}\Delta_i T_i(T)\\
%     \le& \sum_{i\notin D,i\neq i^*} \Delta_i \bracket{ \tau_i + \sqrt{ 4\tau_i \log \frac{T}{\delta} + 5\log^2 \frac{T}{\delta}} } \\
%     &+ \sum_{i\in D,i\neq i^*} \Delta_i\bracket{ \tau_i+ \sum_{s=1}^{\tau_i^D}\gamma_s  +\sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s}+  \sqrt{ 4\bracket{ \tau_i + \sum_{s=1}^{\tau_i^D}\gamma_s + \sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s} }\log \frac{T}{\delta} + 5\log^2 \frac{T}{\delta} } } \,,
% \end{align*}
% where the inequality holds according to Lemma \ref{lem:sto:pullTime}.
% \paragraph{Bound $\tau_i$: }
% At time $\tau_i-1$, it holds that
% \begin{align*}
%     &\Delta_i - 2\sqrt{ \frac{4|D|}{(\tau_i-1)^2} \sum_{s=1}^{\tau_i - 1} \frac{1}{\gamma_s} \log\frac{\tau_i}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i - 1}^2 (\tau_i - 1)^2}\log^2 \frac{\tau_i}{\delta} }\\
%     \le& \tilde{H}_{\tau_i-1}(i^*)-\tilde{H}_{\tau_i-1}(i) \\
%     \le& \max_{j\in A_{\tau_i-1}}\tilde{H}_{\tau_i-1}(j)-\tilde{H}_{\tau_i-1}(i)\\ \le& 6\sqrt{ \frac{4|D|}{(\tau_i-1)^2} \sum_{s=1}^{\tau_i - 1} \frac{1}{\gamma_s} \log\frac{\tau_i}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i - 1}^2 (\tau_i - 1)^2}\log^2 \frac{\tau_i}{\delta} } \,,
% \end{align*}
% where the first inequality comes from Lemma \ref{lem:key:concen} and the second inequality holds according to Lemma \ref{lem:sto:neverDeleteOptimal}. 
% The last inequality above implies that $\tau_i \le \frac{|D|}{K}\bracket{ \frac{1024\log T/\delta}{\Delta_i^2} }^{3/2}$. 

% \paragraph{Bound $\tau_i^D$ for $i\in D$: }
% According to Algorithm \ref{alg}, for each arm $i\in D$, if $i^*\notin N^{\mathrm{out}}(i)$,
% \begin{align*}
%     \tau_i^D =  \max_{j: j\in N^{\mathrm{out}}(i)}\tau_j  \le \max_{j: j\in N^{\mathrm{out}}(i)} \frac{|D|}{K}\bracket{ \frac{1024\log T/\delta}{\Delta_j^2} }^{3/2}\,.
% \end{align*}
% And If $i^*\in N^{\mathrm{out}}(i)$, 
% \begin{align*}
%     \tau_i^D= \max_{j: j\neq i^*}\tau_j 
%     \le \max_{j: j\neq i^*} \frac{|D|}{K}\bracket{ \frac{1024\log T/\delta}{\Delta_j^2} }^{3/2}
% \end{align*}

% \paragraph{Bound $\sum_{s=1}^{\tau_i^D} \gamma_s$ for $i\in D$: }
% \begin{align*}
%     \sum_{s=1}^{\tau_i^D} \gamma_s = \sum_{s=1}^{\tau_i^D} (K^2 |D|)^{1/3}s^{-1/3} \le& K^{2/3}|D|^{1/3} \bracket{ 1+\int_{1}^{\tau_i^D} s^{-1/3}ds } \\
%     \le& K^{2/3}|D|^{1/3} \bracket{ 1+(\tau_i^D)^{2/3} } \\
%     \le& K^{2/3}|D|^{1/3} + |D|\cdot \max_{j:j\neq i^*}\frac{1024\log T/\delta}{\Delta_j^2} \,.
% \end{align*}

% \paragraph{Bound $\sum_{s=\tau_i^D}^{T} \frac{\gamma_s \tau_i^D}{s}  $ for $i\in D$: }

% \begin{align*}
%     \sum_{s=\tau_i^D}^{T} \frac{\gamma_s \tau_i^D}{s} \le \tau_i^D \sum_{s=\tau_i^D}^{T} \frac{\gamma_s}{s} \le& K^{2/3}|D|^{1/3} \tau_i^D \sum_{s=\tau_i^D}^{T} s^{-4/3} \\
%     % \le& K^{2/3}|D|^{1/3}\tau_i^D \bracket{ 1+(\tau_i^D)^{-1/3} } \\
%     \le& 4 K^{2/3}|D|^{1/3}\tau_i^D \,.
% \end{align*}
% Above all, the regret can be bounded by 
% \begin{align*}
%     Reg(T) \le& ~O\left( \sum_{i\neq i^*}\Delta_i \cdot \frac{|D|}{K}\bracket{ \frac{\log T/\delta}{\Delta_i^2} }^{3/2} \right. \\
%     &\left. ~~~~~~~+ \sum_{i\in D,i\neq i^*} \Delta_i \cdot \bracket{ K^{2/3}|D|^{1/3} + |D|\cdot \max_{j:j\neq i^*}\frac{\log T/\delta}{\Delta_j^2} +\max_{j: j\neq i^*} \frac{|D|^{4/3}}{K^{1/3}}\bracket{ \frac{\log T/\delta}{\Delta_j^2} }^{3/2} } \right)\\
%     \le &~ O\bracket{ \frac{|D|^{7/3}}{K^{1/3}} \max_{j:j\neq i^*}\bracket{ \frac{\log T/\delta}{\Delta_j^2} }^{3/2}  } \le O\bracket{ |D|^2 \max_{j:j\neq i^*}\bracket{ \frac{\log T/\delta}{\Delta_j^2} }^{3/2}  } \,.
% \end{align*}


% \end{proof}




% \begin{lemma}\label{lem:sto:pullTime}
% At any time $t=1,2\ldots$, with probability at least $1-\delta$, for each arm $i\in V\setminus D$
% \begin{align*}
%     T_i(t) \le \tau_i + \sqrt{ 4\tau_i \log \frac{T}{\delta} + 5\log^2 \frac{T}{\delta} }\,,
% \end{align*}
% and for each arm $i\in D$,
% \begin{align*}
%     T_i(t) \le \tau_i+ \sum_{s=1}^{\tau_i^D}\gamma_s +\sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s}+  \sqrt{ 4\bracket{ \tau_i + \sum_{s=1}^{\tau_i^D}\gamma_s + \sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s} }\log \frac{T}{\delta} + 5\log^2 \frac{T}{\delta} }
% \end{align*}

% \end{lemma}

% \begin{proof}
% For consistency, for each arm $i\in V \setminus D$, we set $\tau_i^D = 0$. Let $Z_{s,i}(p)\sim \mathrm{Bernoulli}(p)$ for time $s=1,2\ldots,t$, $i\in V$. Then for each arm $i\in V$ and time $t$, 
% \begin{align*}
%     T_i(t) = \sum_{s=1}^t Z_{s,i}(p_{s}(i)) 
%     =  \sum_{s=1}^t Z_{s,i}\bracket{ (1-\gamma_s)\cdot p_{s,A}(i) + \gamma_s \cdot p_{s,D}(i) }\,.
% \end{align*}
% Define $X_{s}(i) = Z_{s,i}(p_{s}(i)) - p_{s}(i) $. We have $\abs{X_{s}(i)} \le 1$ and 
% \begin{align*}
%     \sum_{s=1}^t \EE{X_{s}(i)^2 \mid \cF_{s-1} } \le& \sum_{s=1}^{\tau_i}(1-\gamma_s)\cdot p_{s,A}(i) + \sum_{s=1}^{\tau_i^D} \gamma_s \cdot p_{s,D}(i) + \sum_{s=\tau_i^D}^t \gamma_s\cdot \frac{u_i\tau_i^D}{s} \\
%     \le& \tau_i + \sum_{s=1}^{\tau_i^D}\gamma_s + \sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s} \,.
% \end{align*}
% According to Lemma \ref{lem:tech:concen}, with probability at least $1-\delta$, 
% \begin{align*}
%     \sum_{s=1}^t X_{s}(i) \le \sqrt{ 4\bracket{ \tau_i + \sum_{s=1}^{\tau_i^D}\gamma_s + \sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s} }\log \frac{T}{\delta} + 5\log^2 \frac{T}{\delta} }
% \end{align*}
%  and further
% \begin{align*}
%     T_i(t) \le \tau_i + \sum_{s=1}^{\tau_i^D}\gamma_s + \sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s} + \sqrt{ 4\bracket{ \tau_i + \sum_{s=1}^{\tau_i^D}\gamma_s + \sum_{s=1}^{\tau_i^D}\gamma_s\frac{\tau_i^D}{s} }\log \frac{T}{\delta} + 5\log^2 \frac{T}{\delta} } \,.
% \end{align*}


% \end{proof}









% \begin{lemma}\label{lem:sto:neverStartExp}
% In the stochastic setting, Eq.\eqref{eq:alg:detect:adv} is never satisfied and the Exp3.G algorithm is never started. 
% \end{lemma}

% \begin{proof}
% According to Algorithm \ref{alg}, for each arm $i$, at time $\tau_i$, 
% \begin{align}
%     \max_{j\in A_{\tau_i}}\tilde{H}_{\tau_i}(j) - \tilde{H}_{\tau_i}(i) > 6 \sqrt{\frac{4|D|}{\tau_i^2} \sum_{s=1}^{\tau_i} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i}^2 {\tau_i}^2}\log^2 \frac{{T}}{\delta}  } \,.\label{eq:sto:noadv:1}
% \end{align}
% Besides, according to Lemma \ref{lem:key:concen}, 
% \begin{align}
%     \max_{j\in A_{\tau_i}}\tilde{H}_{\tau_i}(j) - \tilde{H}_{\tau_i}(i) \le& \mu_j - \mu_i + \radius_{\tau_i}(j) + \radius_{\tau_i}(i) \notag \\
%     =&  \mu_j - \mu_i + 2\sqrt{\frac{4|D|}{\tau_i^2} \sum_{s=1}^{\tau_i} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i}^2 {\tau_i}^2}\log^2 \frac{{T}}{\delta}  } \label{eq:sto:since:noadv:notDelete}\\
%     \le& \Delta_i + 2\sqrt{\frac{4|D|}{\tau_i^2} \sum_{s=1}^{\tau_i} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i}^2 {\tau_i}^2}\log^2 \frac{{T}}{\delta}  } \label{eq:sto:noadv:2}
% \end{align}
% where Eq.\eqref{eq:sto:since:noadv:notDelete} holds since $\tau'_{j}\ge \tau_i$ and $\tau'_{i}\ge \tau_i$ when $j\in A_{\tau_i}$ in Algorithm \ref{alg}. 

% Combining Eq.\eqref{eq:sto:noadv:1} and \eqref{eq:sto:noadv:2}, we have
% \begin{align*}
%     \Delta_i > 4\sqrt{\frac{4|D|}{\tau_i^2} \sum_{s=1}^{\tau_i} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i}^2 {\tau_i}^2}\log^2 \frac{{T}}{\delta}  } \,.
% \end{align*}
% Further, according to Lemma \ref{lem:key:concen}, at any time $t$, for any arm $i \notin A_t$,
% \begin{align}
%     \max_{j\in A_{t}}\tilde{H}_{t}(j) - \tilde{H}_{t}(i) \ge \tilde{H}_{t}(i^*) - \tilde{H}_{t}(i) 
%     \ge& \Delta_i - \radius_{t}(i^*) - \radius_t(i)  \notag\\
%     >& 4\sqrt{\frac{4|D|}{\tau_i^2} \sum_{s=1}^{\tau_i} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i}^2 {\tau_i}^2}\log^2 \frac{{T}}{\delta}  } - \radius_{t}(i^*) - \radius_t(i) \notag \\
%     \ge& 2\sqrt{\frac{4|D|}{\tau_i^2} \sum_{s=1}^{\tau_i} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i}^2 {\tau_i}^2}\log^2 \frac{{T}}{\delta}  }  \label{eq:sto:since:valueOfRadius1} \\
%     \ge& \radius_{t}(i^*) + \radius_t(i) \label{eq:sto:since:valueOfRadius2} \,,
% \end{align}
% where Eq.\eqref{eq:sto:since:valueOfRadius1} and \eqref{eq:sto:since:valueOfRadius2} is due to $\radius_t(j) \le \sqrt{\frac{4|D|}{\tau_i^2} \sum_{s=1}^{\tau_i} \frac{1}{\gamma_s} \log\frac{T}{\delta} +\frac{5|D|^2}{\gamma_{\tau_i}^2 {\tau_i}^2}\log^2 \frac{{T}}{\delta}  }  $ for $j=i,i^*$ and $t>\tau_i$. 


% If $i^* \in \argmax_{j \in A_t}\tilde{H}_{t}(j)$, then we have proved Eq.\eqref{eq:alg:detect:adv} is not satisfied at time $t$. Otherwise if $\exists j' \neq i^*$ and $j' \in \argmax_{j \in A_t}\tilde{H}_{t}(j)$, it holds that $\tau'_{j'}>t$, $\tau'_{i^*}>t$ and $\radius_{t}(i^*) = \radius_{t}(j')$. Thus 
% \begin{align*}
%     \max_{j\in A_{t}}\tilde{H}_{t}(j) - \tilde{H}_{t}(i) = \tilde{H}_{t}(j') - \tilde{H}_{t}(i) >  \radius_{t}(j') +  \radius_{t}(i)\,,
% \end{align*}
% and Eq.\eqref{eq:alg:detect:adv} is still not satisfied. 
% \end{proof}





% \begin{lemma}\label{lem:sto:neverDeleteOptimal}
% At any time $t$, $i^*\in A_t$. 
% \end{lemma}
% \begin{proof}
% At any time $t$, for any arm $j \in A_t$, we have
% \begin{align}
%     \tilde{H}_{t}(j) - \tilde{H}_{t}(i^*) \le& \mu_j - \mu_{i^*} + \radius_t(i)+ \radius_{t}(i^*) \label{eq:sto:since:radius} \\
%     =& \mu_j - \mu_{i^*} + 2\sqrt{\frac{4|D|}{t^2} \sum_{s=1}^t \frac{1}{\gamma_s} \log\frac{t}{\delta} +\frac{5|D|^2}{\gamma_t^2 t^2}\log^2 \frac{t}{\delta}  } \label{eq:sto:since:notDelete} \\
%     =& -\Delta_j + 2\sqrt{\frac{4|D|}{t^2} \sum_{s=1}^t \frac{1}{\gamma_s} \log\frac{t}{\delta} +\frac{5|D|^2}{\gamma_t^2 t^2}\log^2 \frac{t}{\delta}  }\notag \\
%     \le & 6\sqrt{\frac{4|D|}{t^2} \sum_{s=1}^t \frac{1}{\gamma_s} \log\frac{t}{\delta} +\frac{5|D|^2}{\gamma_t^2 t^2}\log^2 \frac{t}{\delta}  } \,, \notag
% \end{align}
% where Eq.\eqref{eq:sto:since:radius} comes from Lemma \ref{lem:key:concen}, Eq.\eqref{eq:sto:since:notDelete} holds since $\tau'_{j}>t$ and $\tau'_{i^*}>t$ when both $j,i^*\in A_t$. 

% \end{proof}





